Physiological Tremor Increases when Skeletal Muscle is Shortened: Implications for Fusimotor Control

The involuntary force fluctuations associated with physiological (as distinct from pathological) tremor are an unavoidable component of human motor control. While the origins of the physiological tremor are known to depend on muscle afferentation, it is possible that the mechanical properties of muscle-tendon systems also affect its generation, amplification and maintenance. In this paper, we investigated the dependence of physiological tremor during tonic, isometric plantarflextion torque at 30% of maximum at three ankle angles. The amplitude of physiological tremor increased as calf muscles shortened in contrast to the stretch reflex whose amplitude decreases as muscle shortens. We used a closed-loop simulation model of afferented muscle to explore the mechanisms responsible for this behavior. We demonstrate that changing muscle lengths does not suffice to explain our experimental findings. Rather, the model consistently required the modulation of gamme-static fusimotor drive to produce increases in physiological tremor with muscle shortening--while successfully replicating the concomitant reduction in stretch reflex amplitude. This need to control gamma-static fusimotor drive explicitly as a function of muscle length has important implication. First, it permits the amplitudes of physiological tremor and stretch reflex to be decoupled. Second, it postulates neuromechanical interaction that require length-dependent gamma drive modulation to be independent from alpha drive to the parent muscle. Lastly, it suggests that physiological tremor can be used as a simple, non-invasive measure of the afferent mechanisms underlying healthy motor function, and their disruption in neurological conditions.

==> reviews.tex <==
\begin{question}
any recent study on tremor and its modulation with muscle length or stretch reflex? If no, mention this.  Give some background on what is known about tremor and why is it important to study this. 
\end{question}
\begin{response}
We changed the first paragraph of introduction to express that this relationship has not been previously characterized. This is one of the key findings of the paper (mentioned in keypoint summary, abstract, result, discussion). We also further clarified this in the introduction now.
\end{response}
\begin{question}
Why did you choose plantarflexor muscles? you might want to explain that you choose these muscles bcs you were interested to find the correlation between reflex response (muscle stretch) and tremor; the reflexes are very small in dorsiflexors.
\end{question}
\begin{response}
We have added reasons for using the plantarflexor muscles in the introduction now.
\end{response}

\begin{question}
Figure 1: is it possible to add a vertical line to show the neutral position?
\end{question}

\begin{response}
I have made an attempt to a vertical line but it was difficult to interpret visually as it needed extra text for explanation. I also tried adding another ankle joint at the neutral position but it did not look good either. So, I decided to remove it the neutral position all together.

Nevertheless, I added the description of neutral position in the figure caption as well as in the method section.

\end{response}
\begin{question}
This way of referring to the thy three positions is awkward. Can you not define them in a simpler manner e.g PF,mid,DF
\end{question}
\begin{response}
Figures and text are now revised to PF, MID, DF.
\end{response}
\begin{question}
What are the properties of the SDN?
\end{question}
\begin{response}
The properties of the SDN are now explained in the methods section.
\end{response}
\begin{question}
Model: 30ms delay for monosynaptic reflex seems short.
\end{question}
\begin{response}
This was a mistake. We examined the delay again and it was approximately 35ms. We have revised to text to reflect this.
\end{response}

\begin{question}
so is 30s for experimental data enough?
\end{question}
\begin{response}
It was 90s not 30s because we recorded 3x30 s (see methods). 90 s should be enough for a PSD analysis.
\end{response}

\begin{question}
Methods: Clarify whether Were the gamma drives were changed independently or in synchrony
\end{question}
\begin{response}
We changed them independently. text revised and clarified.
\end{response}

\begin{question}
Key finding. Need to demonstrate that alpha drive was invariant
\end{question}

\begin{response}
We have revised the paper and added a new figure to demonstrate this.
\end{response}

\begin{question}
Figure 4 should indicate statistically significant changes.
\end{question}
\begin{response}
Done!
\end{response}
\begin{question}
on the use of gastrocnemius muscle: This analysis is flawed since torque may be correlated with the activity of the other muscles as well. you have no indication of how much of the torque variance is accounted for by the gastroc EMG. The other muscles of the triceps surae could also be contributing significantly.
\end{question}
\begin{response}
We agree that other muscles also contribute to the torque and might be equally important in torque generation. However, here the focus is \emph{not} on which muscle contributes more to the torque but rather to identify the muscle that is more coherent with the torque in the physiological tremor band (5-12 Hz) and then use that muscle for the simulation study. It turns out that the coherence of the Medial head of the gastroc muscle in the tremor band always larger than the significance threshold compared to other muscles. Again, since we did not want to use a highly complicated multi-muscle model, we had to select only one muscle. Based on the experimental data, we chose the medial head of the gastrocnemius as this was the most coherent in the tremor band. We revised the method and result section to address this concern.
\end{response}
\begin{question}
Two problems here. You repeated talk about a inverse relation of tremor power with muscle length and that is certainly what it looks like in Fig 2. However, according to the results presented in Section 4.4. the only difference you demonstrated is that that tremor is great at 20PF than the other two positions. This makes you reliance on the systematic change doubtful. Ideally it would have been better to have measurements at more positions.


As an aside where do these positions fit w,r.t the ROM. Are they both about the same distance from the end ?
\end{question}
\begin{response}
1) There was a problem with the way we set up our statistical test. So, we revisited this analysis. We found the tremor in the PF position was significantly larger than MID and DF positions. We also found that the tremor in the MID position was significantly larger than DF position. We revised the paper accordingly.

2) We did not select the position angles based on the subject ROM. they were absolute positions based on the neutral position symmetric around the MID position.
\end{response}
\begin{question}
I think you needed to show the equivalent of figure 2 for the simulation results to convince the reader that your simulations are realistic
\end{question}
\begin{response}
Done! New Figure 4.
\end{response}
\begin{question}
So how does the increased static drive increase tremor if the reflex gain decreases.
\end{question}
\begin{response}
Discussion is now revised to address this. In a previous publication (Jalaleddini et al, JNE, 2017) we have shown that increased static drive actually decreases the phasic reflex response and the thus the reflex gain.
\end{response}

\begin{question}
in discussion: ``Even with these limitations, our prediction of neural (rather than purely mechanical) responses
to altered muscle length remains a valid and perhaps even the most straight-forward explanation
for our experimental observations.''

This is a strong claim that needs to be supported more clearly
\end{question}
\begin{response}
Agreed and revised.
%{\color{red}@AKIRA@CHRIS I agree that this is a strong claim. I think we should soften it. Do you agree? ..... chriscomment: Maybe just say a valid and particularly straight-forward explanation.... rather than THE most straight-forward}
\end{response}
\begin{question}
The failure to measure muscle stiffness and reflex response experimentally weakens the argument.
\end{question}
\begin{response}
Mahsa tested one subject for stiffness and stretch reflex and the pattern was consistent with the previous reports. We added a section under the Results to address this. The findings are consistent with the one from the model and those reproduced from previous experimental results.
\end{response}
\begin{question}
As a read it you only explored one amplitude of pre-synaptic inhibition.  What happens if you increase the amplitude of the change. Another possibility might be co-activation of TA as GS was shortened and TA lengthened. Was TA EMG measured to rule this out?
\end{question}
\begin{response}
We did measure the TA EMG. We calculated the RMS of the EMG at the three positions and found that there was no consistent pattern in activation of the TA. This possibility is now explored and addressed in the paper (methods and results revised).
\end{response}
\begin{question}
You repeatedly mention that muscle stiffness decreases as you go from DF to PF. In fact it is a “U” shaped relation where stiffness  decreases as you go from DF to the mid range and then increases as you continue to PF. Are you sure that you are in the flat region.
\end{question}
\begin{response}
Correct. Stiffness has a U shape. However, since the U shape is skewed toward plantarflexed positions (i.e. the minimum is at a plantarflexed position of around -0.45 rad) and the positions that we tested were all located on one side of the U shape (tested positions were all larger than -0.45rad), stiffness is monotonically increasing with dorsiflexion. We revised the paper to address this comment (results and discussion revised).
\end{response}
